AI-lead Court Debate Case Investigation

The multi-role judicial debate composed of the plaintiff, defendant, and judge is an important part of the judicial trial. Different from other types of dialogue, questions are raised by the judge, The plaintiff, plaintiff's agent defendant, and defendant's agent would be to debating so that the trial can proceed in an orderly manner. Question generation is an important task in Natural Language Generation. In the judicial trial, it can help the judge raise efficient questions so that the judge has a clearer understanding of the case. In this work, we propose an innovative end-to-end question generation model-Trial Brain Model (TBM) to build a Trial Brain, it can generate the questions the judge wants to ask through the historical dialogue between the plaintiff and the defendant. Unlike prior efforts in natural language generation, our model can learn the judge's questioning intention through predefined knowledge. We do experiments on real-world datasets, the experimental results show that our model can provide a more accurate question in the multi-role court debate scene.

==> 6_Related_work.tex <==
\section{Related work}
\subsection{Legal Intelligence}
LegalTech(legal technology) is not a new concept that was put forward in 1960s\cite{nagel1960using}. Since then a lot of researcher from both law and computer science fields have been exploring the potential and methods to predict judicial decisions or auxiliary tasks, aiming at helping lawyers and lower court judges. In the recent work, Zhou et al. leveraged multi-view dispute representation for predicting e-commerce judge result\cite{zhou2019legal}. Oard et al. studied the information retrieval for e-discovery \cite{oard2010evaluation,oard2013information}. Wang et al. \cite{wang2018modeling} proposed a model for crime classification. Wang et al. \cite{wang2019hierarchical}leveraged fact, law and artical information to build a hierarchical matching network for crime classification. Megala et al. \cite{megala2014feature} and Polsley et al. \cite{polsley2016casesummarizer} proposed several statistics-based methods (e.g., TFIDF) and some manually defined features to extract important part of the document for legal text summarization task.

Compared to all the prior efforts in NLG, this study can be novel in the following aspects. First, our work is generating questions at each turn for judges in court debate scenario during trial procedure. The multi-role debate are much more complicated but extremely important due to the vague/informal expressions conveyed through dialogues and the frequent switch among the speakers, which undoubtedly makes the understanding and the learning process much challenging. Second, the keyword or simple statistics-based methods are not suitable to address this problem because of its diverse expressions of spoken language compared to written language. In this study, we pioneer this problem by encoding the contextual utterance information with respect to global legal knowledge and local case judicial factors, as well as simulating the intention switch across different conversation turns. 


% \subsection{Dialogue System}
% In recent years, the research of dialogue system has developed vigorously.
% Many new tasks have been proposed: a VGDS is proposed to generate the most appropriate response based on video content, video title, and existing conversation statements \cite{le2019multimodal};
% Tang et al. proposed  a conversational system to chat naturally with human and proactively guide the conversation to a designated target subject\cite{tang2019target};
%  Wang et al. proposed how to use different persuasion strategies in the conversation to persuade people to donate to charity\cite{wang2019persuasion}.

% Many novel dialogue generation work using specific knowledge graph is also endless: Liu et al. propose a neural knowledge diffusion (NKD) model to introduce knowledge into dialogue generation. This method can not only match the relevant facts for the input utterance but diffuse them to similar entities\cite{liu2018knowledge};
% Williams et al. introduce Hybrid Code Networks (HCNs), which combine a RNN with domain-specific knowledge encoded as software and system action templates\cite{williams2017hybrid};
% Wu et al. uses the mark triplet to obtain the link between the dialogues\cite{wu2019proactive}; Moon et al. proposes a graph decoder based on the attention mechanism\cite{moon2019opendialkg}; Zhou et al. attempts to use the large-scale common sense knowledge graph to handle conversation generation problems\cite{zhou2018commonsense}.

% In this work we introduce a novel methodology to assist judges to lead the court debate. Different from other dialog systems above, in a multi-role court debate judges only ask questions to plaintiff, defendant, and witness rather than answer questions.



\subsection{Question Generation}
Question generation is a very important task in the field of NLP, which is widely used, including question answering systems, dialogue system and intelligent tutoring systems.
So far, researchers have done a lot of research work on question generation.
Tang et al.takes question generation and reading comprehension as dual tasks to joint training\cite{tang2017question}. Wang et al. also combine question generation(QG) with question answering(QA), while treating both QG and QA as generation tasks. Du et al.\cite{du2017identifying} first use the classifier to select a sentence related to the question from the article to further generate the question\cite{wang2017joint}. Guo et al. adopt multi-task learning method, use question generation and implication generation to assist summary generation task\cite{guo2018soft}.
Elsahar et al. proposed Zero-Shot generation model and use the knowledge graph triples as input to generate questions\cite{elsahar2018zero}.

In this work, we propose a question generation model for the court debate scene by not only use multi-role debate context information but also leveraging Legal Knowledge Graph and intent navigation.
